Collisional radiative modelling with improved cross sections to investigate plasma molecular interactions in divertor plasmas

Power exhaust is one of the main challenges for the realization of practical fusion energy production. The magnetic confinement approach to fusion often uses a divertor configuration, where power loads are critical. Recent SOLPS simulations of divertor plasmas in MAST-U and TCV show significant deviations from the experimental results [36, 35]. A possible explanation for this is the incorrect incorporation of plasma-molecular interactions in current SOLPS simulations. SOLPS uses tabulated rate data for the particle physics part of the simulations [37, 23]. There are, however, large concerns about the accuracy of these rates, especially for plasma-molecular interactions [33]. Therefore, in this work, improved rate data from different sources, such as the Laporta[18] and MCCCDB[29, 27, 28] databases was used, to construct a Collisional Radiative Model (CRM) to investigate the plasma molecular interactions in conditions relevant to the MAST-U Super-X divertor. It was shown that using these rates, a better correspondence with experiment is achieved than with the tabulated rates. In particular, increased Molecular Activated Recombination (MAR) and Dissociation (MAD) was observed. Additionally it was found that molecular processes may be a significant contributor to divertor physics. The effect of different processes on the vibrational distribution was also investigated, as well as the radiative emission spectra generated from the CRM. It was demonstrated that re-evaluation of reaction rates for plasma-molecular interactions in plasma-edge modelling is necessary.

==> Interim_results.tex <==

\section{Interim results 1-5-2023}
In this section, I will present the results I obtained in the first week of my internship at UKAEA. 

The goal this first week was to use a fast Collisional Radiative Model (CRM) such as CRUMPET to calculate effective rates for a few different reactions, starting with molecular charge exchange. 

\begin{equation}
    \text{p}+\text{H}_2(\nu) \rightarrow \text{H}+ \text{H}_2^+
    \label{eq:mol_cx}
\end{equation}

The molecular hydrogen is in a certain vibrational state $\nu$. It is important to track these states, because the reaction rates depend on the vibrational state of the hydrogen molecule. The CRM I used takes the first 15 states (i.e. the ground state $\nu=0$ and 14 excited states) into account. Given the reaction rates for the different vibrational states, CRUMPET can calculate the vibrational distribution. The effective reaction rate can then be calculated by summing the different rates, weighted by the vibrational distribution. 

\begin{equation}
    \langle\sigma v\rangle_{eff} = \sum^{14}_{\nu=0} f_\nu \langle\sigma v\rangle_\nu
    \label{eq:eff_rate}
\end{equation}

Here, $f_\nu$ is the fraction of hydrogen molecules that are in vibrational state $\nu$, $\langle\sigma v\rangle_\nu$ is the reaction rate of state $\nu$, and $\langle\sigma v\rangle_{eff}$ is the effective reaction rate. 

The rates $\langle\sigma v\rangle_\nu$ are taken from two different sources. The first is the H2VIBR database, which was probably used to calculate the effective rates that are currently in the HYDHEL database. Alternatively, the rates can be obtained using data from a paper by Ichihara et al. from 2000. They did an exhaustive quantum mechanical calculation to obtain rates for temperatures below 20 eV. Because both $f_\nu$ and $\langle\sigma v\rangle_\nu$ depend on temperature, the effective rates will also depend on temperature. 

Firstly I calculated the vibrational distribution and effective rates of molecular charge exchange (equation \eqref{eq:mol_cx}), dissociation (equation\eqref{eq:dissociation}), and ionization (equation \eqref{eq:ionization}), using the H2VIBR vibrationally resolved rates, and compared them to the HYDHEL effective rates. The vibrational distribution and effective reaction rates are given in \autoref{fig:H2VIBR}. Note that for fusion applications, the reactions will involve deuterium, not hydrogen. This does not matter for ionization and dissociation, but it does for charge exchange. In this case, the temperature must be scaled with the isotope mass. 

\begin{equation}
    e+\text{H}_2(\nu)\rightarrow e+2\text{H}
    \label{eq:dissociation}
\end{equation}

\begin{equation}
    e+\text{H}_2(\nu)\rightarrow 2e+\text{H}_2^+
    \label{eq:ionization}
\end{equation}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/vibr_distr_h2vibr.png}
         \caption{}
         \label{fig:vibr_distr_h2vibr}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/reactions.png}
         \caption{}
         \label{fig:H2VIBR}
     \end{subfigure}
        \caption{Vibrational distribution and effective reaction rates using H2VIBR rates. The effective rates are compared to the standard HYDHEL rates. In (a), the different lines represent the fractional abundance of different vibrational states.}
        \label{fig:three graphs}
\end{figure}

Eventually, we would like to use the calculated effective rates in models like SOLPS. It is therefore convenient to store the data in a similar format to the AMJUEL database. This database is a LaTeX file, containing 8th order logarithmic fit constants of the effective rates as a function temperature. The fit coefficients $b_i$ are defined as:

\begin{equation}
    \ln(\langle\sigma v\rangle_{eff}) \approx b_0 + b_1 \ln(T) + b_2 (\ln(T))^2 + ... + b_8 (\ln(T))^8
\end{equation}

The fit coefficients for molecular charge exchange for example are:

\begin{small}\begin{verbatim}
  b0 -2.485405296479D+01  b1  9.124837134392D+00  b2 -8.603038604800D+00
  b3  2.696948087189D+00  b4 -1.640190821543D-01  b5  1.154721025377D-02
  b6 -3.964741081497D-02  b7  1.106164075808D-02  b8 -8.773682376758D-04
\end{verbatim}\end{small}

We can also use the Ichihara et al. data to calculate the vibrational distribution and effective rates. CRUMPET also uses LaTeX files containing fit constants as input. So the Ichihara rates must be fitted first, and the constants put into the H2VIBR file as separate entries. We can then  use these data as the new reaction rates for molecular charge exchange and calculate the vibrational distribution. Because the Ichihara rates are only defined below 20 eV, we had to extrapolate the data such that the fit constants produce accurate results for higher temperatures. The vibrationally resolved rates, as well as the new vibrational distribution is given in \autoref{fig:Ichihara}.


\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/rates_ichihara.png}
         \caption{}
         \label{fig:rates_ichihara}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
        \includegraphics[width=\textwidth]{Pictures/vibr_distr_ichihara.png}
        \caption{Vibrational distribution using Ichihara rate data. }
        \label{fig:vibr_distr_ichihara}
     \end{subfigure}
        \caption{Vibrationally resolved rates and the resulting vibrational distribution for Ichihara data. }
        \label{fig:Ichihara}
\end{figure}

Finally, the effective reaction rate for molecular charge exchange can be calculated using Ichihara data. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Pictures/Charge_exchange.png}
    \caption{Effective rates for molecular charge exchange, calculated using H2VIBR and Ichihara data.}
    \label{fig:Charge_exchange}
\end{figure}

\section{Interim results 8-5-2023}
The next step to improving the accuracy of the CRM is to use accurate cross sections from different sources for all the reactions in the model. The reactions and their respective databases are in \autoref{tab:rea_ref}. You can see that also electronically excited states are added to the model. 

First, we will inspect the difference of the steady state vibrational distribution between the previously used H2VIBR rates and `the new cross sections from Laporta et al.. Laporta did quantum mechanical calculations using the R-matrix method to obtain cross sections for a large number of different reactions. Additionally, the Laporta database contains cross sections for excitation between all 15 states. The H2VIBR database only contains excitation and deexcitation of one level up or down at a time. Laporta does not have cross sections for deexcitation, however. These can be calculated using the principle of detailed balance, which assumes the following relation for the cross sections: 
\begin{equation}
    \sigma_{deex}(T) = \sigma_{ex}(T)e^{-\frac{\Delta E}{k_BT}} 
    \label{eq:det_balance}
\end{equation}

The vibrational distributions for the case that only direct vibrational transitions are taken into account are given in \autoref{fig:Distr_vibr_only}. You can see a clear difference between the older data and the newly aqcuired Laporta data. The fractional abundance of the vribrationally excited states at low temperature are much higher using the new data. Physically, this means that even at low temperatures (such as in a MAST-U super-X divertor) the vibrationally excited states will play a larger role. 

\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/Distr_vibr_only_old.png}
         \caption{H2VIBR}
         \label{fig:Distr_vibr_only_old}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
        \includegraphics[width=\textwidth]{Pictures/Distr_vibr_only.png}
        \caption{Laporta}
        \label{fig:Distr_vibr_only_new}
     \end{subfigure}
        \caption{Vibrational distributions as function of temperature, calculated using H2VIBR (a) and Laporta cross sections (b).}
        \label{fig:Distr_vibr_only}
\end{figure}


The detailed balance cross sections also give us a method to test the CRM. If we put in the Laporta data for excitation, and use detailed balance for the deexcitation data, the CRM should simply produce a Bolzmann distribution, given in equation \eqref{eq:bolzmann}. \autoref{fig:Bolzmann} demonstrates that this is indeed the case.

\begin{equation}
    N_v = Cg_\nu e^{-\frac{E}{k_BT}}
    \label{eq:bolzmann}
\end{equation}

\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/Bolz_dev_vibr_only.png}
         \caption{}
         \label{fig:Bolz_dev}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
        \includegraphics[width=\textwidth]{Pictures/Vibr_fit_T.png}
        \caption{}
        \label{fig:Vibr_fit_T}
     \end{subfigure}
        \caption{This figure serves to compare the vibrational distribution, calculated with only the Laporta data for vibrational (de-)excitation, to a Bolzmann distribution (see equation \autoref{eq:bolzmann}. (a) contains a plot of the deviation of the distribution from a Bolzmann as a function of temperature. You can see that the distribution is particularly close to a Bolzmann distribution for high temperatures. (b) contains a plot of the distribution at a certain temperature.}
        \label{fig:Bolzmann}
\end{figure}

Here, $N_{\nu}$ is the number density of a particular vibrational state $\nu$, C is a constant, $g_\nu$ is the degeneracy of the state (which in the case of molecular hydrogen is 1), $E$ is the energy level, $T$ is temperature, and $k_B$ is the Bolzmann constant. 



\subsection{More reactions}

Now it's time to add more reactions, and see to what extent the other reactions affect the vibrational distributions. We can also calculate new effective rates using the new MCCCDB and Laporta data. We will first consider the model without electronic excitation. Input file includes vibrational transitions (in the ground state), ionization, dissociation, dissociative ionization, and molecular charge exchange. \autoref{fig:std_new} contains the new vibrational distribution, as well as the newly calculated effective reaction rates. You can see that the fractional abundance of the higher excited states become quite chaotic at higher temperatures. This is possibly due to limitations of the cross-sectional data, but will need further investigation. 

\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/Distr_std_new.png}
         \caption{}
         \label{fig:Distr_std_new}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/Eff_rates_std_new.png}
         \caption{}
         \label{fig:Eff_rates_std_new}
     \end{subfigure}
        \caption{Vibrational distribution and effective reaction rates using Laporta and MCCC cross sections. The effective rates are compared to the standard HYDHEL rates. In (a), the different lines represent the fractional abundance of different vibrational states. The fractional abundance of higher vibrational states seems to become quite chaotic for higher temperatures. This is possibly due to limitations of the temperature range of the data. This is something I still need to figure out. You can also see that the effective rates of the different reactions are quite different from the HYDHEL rates.}
        \label{fig:std_new}
\end{figure}


\subsection{Electronically excited(!) states}
We can also add electronically excited states of molecular hydrogen to the model. We will first consider only the ground state $X^1\Sigma_g$ first two excited states, $B^1\Sigma_u$ and $C^1\Pi_u$. A molecule can be excited by electron collision, and de-excited by radiative decay. We first leave the excited states vibrationally unresolved. This means that we will only consider one kind of molecule per electronically excited state. 

The cross sections for electron collision excitation can simply be obtained from the MCCCDB. The radiative deexcitation rates are a bit more complicated. Even though we don't consider vibrational states in the electronically excited states, it is still important to calculate which vibrational state they radiatively decay into. This can be done by using the so-called Franck-Condon factors, which were calculated for D$_2$ by Fantz et al. in 2006. The rates can be calculated using 

\begin{equation}
    A_\nu = A\cdot FC.
\end{equation}

Here A is total decay frequency of the transition (is also obtained from Fantz), FC is the corresponding Franck-Condon factor, and $A_\nu$ is the decay frequency of the transition into a certain vibrational state $\nu$. Because the Franck-Condon factors are given for the transitions from a vibrationally resolved excited state, they must be averaged over all the vibrational states of the electronically excited state. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Distr_B_C_only.png}
    \caption{Vibrational distribution in the ground state of molecular deuterium. This calculation takes into account only vibrational transitions in the ground state, and excitation to and radiative decay from the first two excited states $B^1\Sigma_u$ and $C^1\Pi_u$. No other reactions were taken into account here, because I wanted to investigate the effect of adding electronically excited states.}
    \label{fig:my_label}
\end{figure}


\subsection{What's next?}
There are some difficulties with the current model that need to be resolved, such as the erratic behaviour of the vibrational distribution at higher temperatures. After that, the effect of reactions including D$^-$ ions can be investigated, such as dissociative attachment. This reaction is expected to have a significant influence at lower temperatures. We can also include emission from the Fulcher band of the deuterium molecules. This would be particularly interesting, because if we can calculate the rate of emission in the Fulcher band, we can directly compare this to experiments. 

Ultimately, the goal will be to create a fully vibrationally resolved model. This means we also have to include vibrational states in the electronically excited states. At this point, we would have a highly sophisticated CRM containing the newest cross-sectional data, and we should be able to calculate highly accurate effective reaction rates for larger 1D or 2D models. 



\begin{table}[H]
\centering
\begin{tabular}{|l|l|l|}
\hline
Reaction                & Formula & Database \\
\hline
 & & \\
Vibrational transitions X$^1\Sigma_u$ & $e+\text{D}_2(\nu=i)\rightarrow e+\text{D}_2(\nu=j)$    &  Laporta/H2VIBR         \\
 & & \\
Dissociative attachment & $e+\text{D}_2(n,\nu)\rightarrow \text{D}^-+\text{D}$       &  Laporta       \\
 & & \\
Dissociative ionization & $e+\text{D}_2(n,\nu)\rightarrow 2e+\text{D}^++\text{D}$ & HYDHEL \\
 & & \\
Ionization & $e+\text{D}_2(n,\nu)\rightarrow 2e+\text{D}_2^+$ & MCCCDB \\
 & & \\
Electronic excitation & $e+\text{D}_2(n=A,\nu=i)\rightarrow e+\text{D}_2(n=B,\nu=j)$ & MCCCDB \\
 & & \\
Radiative deexcitation & $\text{D}_2(n=A,\nu=i)\rightarrow \text{D}_2(n=B,\nu=j) + \hbar\omega$ & Fantz\\
 & & \\
Electron impact dissociation & $e+\text{D}_2(n,\nu)\rightarrow e+2\text{D}$ & MCCCDB \\
 & & \\
\hline
\end{tabular}
\caption{References for reaction data}
\label{tab:rea_ref}
\end{table}


Look at units for reactions because there is a huge difference between tabulated rates and caluclated rates. 

Look for branching ratios in stead of FC factors. 

Hydhel H1 2.2.9 cross sections for H2 ionization from ground 

Give Kevin access to report 

\section{Interim results 15-5-2023}

\subsection{Vibrationally unresolved case}
After further examination of the results of \autoref{fig:Distr_std_new}, it was concluded that CRUMPET possibly has some trouble reliably using MCCC formatted data for its calculations. MCCC provides simply a table containing collision energies and corresponding cross sections. We need logarithmic fit constants of the reaction rate $\langle\sigma v\rangle$ as a function of temperature. Therefore, we must integrate the cross sections over a Bolzmann velocity distribution. 

\begin{equation}
    f(v) = \left(\frac{m}{2\pi k_B T_e}\right)^{3/2}4\pi v^2 e^{\frac{mv^2}{2k_B T_e}}.
    \label{eq:Bolzmann}
\end{equation}

This is the velocity distribution of electrons. Because deuterium molecules are over 7000 times more massive than electrons, their velocity will be negligible compared to that of the electrons. It is therefore sufficient to assume the case of a stationary molecule, hit by an electron at finite velocity. Under this assumption, the reaction rate can be calculated using 

\begin{equation}
    \langle\sigma v\rangle = \int^{\infty}_{0} f(v)v\sigma(v)dv.
\end{equation}

with $v=\sqrt{\frac{2E}{m}}$. 

For some MCCC reactions, the cross sections are only given for low energies, up to around 150 eV. Because of the tail of the Bolzmann distribution, the cross sections of the reaction at higher energies also contributes to the total reaction rate, especially at higher temperatures. The data is therefore extrapolated linearly in loglog space for higher energies. An example of the resulting cross sections is given in \autoref{fig:Ion_examples}. 

\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/Ion_cs_X1_v=0.png}
         \caption{}
         \label{fig:Ion_cs_X1_v=0}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/Ion_sv_X1.png}
         \caption{}
         \label{fig:Ion_sv_X1}
     \end{subfigure}
        \caption{Cross section for D$_2$ ionization from the $X^1\Sigma_u$, $\nu=0$ state (a). The data was extrapolated from 1000 eV onwards. (b) contains the resulting reaction rates as a function of temperature. The different lines represent ionization rates from different vibrational levels. }
        \label{fig:Ion_examples}
\end{figure}

The rates of \autoref{fig:Ion_sv_X1} can be fitted using a logarithmic polynomial fit. The fit constants can then be used to run CRUMPET. This procedure was completed for all the different reactions in \autoref{tab:rea_ref}. The resulting vibrational distribution is given in 


\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/Distr_std_new_fit.png}
         \caption{}
         \label{fig:Distr_std_new_fit}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/Rates_std_new_fit.png}
         \caption{}
         \label{fig:Eff_rates_std_new_fit}
     \end{subfigure}
        \caption{Vibrational distribution and effective reaction rates using Laporta and MCCC cross sections. The effective rates are compared to the standard HYDHEL rates. In (a), the different lines represent the fractional abundance of different vibrational states. You can see that the distribution is now smooth as a function of temperature. Also the effective rates are closer to the HYDHEL rates for higher temperatures. }
        \label{fig:std_new_fit}
\end{figure}

The calculations of \autoref{fig:std_new_fit} include the following reactions:
\begin{itemize}
    \item Vibrational transitions in the $X^1\Sigma_g$ state;
    \item Excitation from $X^1\Sigma_g$ to the $B^1\Sigma_u$ and the $C^1\Pi_u$ states;
    \item Radiative decay from $B^1\Sigma_u$ and $C^1\Pi_u$ to $X^1\Sigma_g$;
    \item Ionization from $X^1\Sigma_g$;
    \item Molecular charge exchange;
    \item Dissociative attachment;
    \item Dissociative excitation.
\end{itemize}

The radiative decay rates were no longer calculated using Franck-Condon factors, but were simply taken from the transition probabilities from Fantz et. al. 

\subsection{Vibrationally resolved case}
Now that last week's problems have been solved, we can take the next step in constructing a physically accurate and useful model: vibrationally resolved excited states. This way, more transitions between different levels can be taken into account. Also, the vibrational distribution can also be calculated in the electronically excited states now. Due to the inclusion of both radiative and collisional processes, the vibrational distribution in the ground state becomes density dependent. For example, a molecule in an excited state can radiatively decay back to the ground state (or another lower energy state), or it can collisionally be ionized. At low electron densities, it is much more likely that the molecule simply decays to a lower state, while ionization becomes more likely at higher densities. Therefore, these multistep processes can result in density dependence. \autoref{fig:Distr_densities} contains vibrational distributions for different 

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/Dist_low_n.png}
         \caption{$n_e=10^{10}$ m$^{-3}$}
         \label{fig:Distr_n=1e10}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/Dist_res_full_1.png}
         \caption{$n_e=10^{19}$ m$^{-3}$}
         \label{fig:n=Distr_1e19}
     \end{subfigure}
        \caption{Vibrational distribution using Laporta and MCCC cross sections, for different electron densities. You can see that for low densities, there is a much higher abundance of vibrationally excited molecules. A possible explanation is that the excited molecules decay into high vibrational states. For higher densities, this is less likely to happen, because electronically excited molecules are ionized before they can decay back to the ground state. }
        \label{fig:Distr_densities}
\end{figure}

\subsection{Planning}
This section contains a rough planning for the coming weeks.

\begin{center}[h]
\begin{tabular}{| p{0.1\textwidth} | p{0.1\textwidth} | p{0.7\textwidth} |}
\hline
Week nr. & Dates     & Explanation of tasks  \\
\hline
\hline
1        & 24/4-30/4 & Getting settled, gaining access to the IT facilities. Calculating effective rates using Ichihara rates for charge exchange and HYDHEL rates for the other reactions. \\                                         
\hline
2        & 1/5-7/5   & Using Laporta, MCCCDB and Fantz to replace data from HYDHEL and add more reactions and excited states to the model.                                                                                                                                                                                                                                                      \\
\hline
3        & 8/5-14/5  & Using cross sectional data from Laporta and MCCCDB to calculate rates as a function of temperature by integrating over a Bolzmann distribution. These rates can in turn be fitted, the constants can be used to run CRUMPET. Also creating the vibrationally resolved model including n=1 and n=2 excited states, as well as the d3 state to calculate Fulcher emission. \\
\hline
4        & 15/5-21/5 & Completing the vibrationally resolved model with all relevant transitions. Begin reading about the Greenland criterion, which can be used to reduce the matrix of the CRM.                                                                                                                                                                                               \\
\hline
5        & 22/5-28/5 & Implementing the Greenland method to reduce the matrix and consequently reducing the computation time.                                                                                                                                                                                                                                                                   \\
\hline
6        & 29/5-4/6  & Model is completely finished. From this moment on, I will be focusing on using the model to do physics. A starting place would be to investigate the emission from d3 to a3 (Fulcher).                                                                                                                                                                                   \\
\hline
7        & 5/6-11/6  & Investigating radiative power losses as a function of  temperature and densities.                                                                                                                                                                                                                                                                                        \\
\hline
8        & 12/6-18/6 & Possibly investigating ionization and dissociation rates and comparing them to experiment. Begin writing the full report.  \\
\hline  
9       & 19/6-25/6 &   Continue writing report, and doing physical calculations\\
\hline
10      & 26/6-2/7  &   Submit first draft of the report + Begin working on presentation \\
\hline
11      & 3/7-9/7 &   Submit final draft of report + give presentation. \\
\hline
\end{tabular}
\end{center}

\section{Interim results 5-6-2023}
\subsection{List of reactions}
In the last few weeks, I've been busy building the model to its current size. The following is a comprehensive list of all the reactions in the final, vibrationally resolved model. All electronically excited states mentioned in the list are vibrationally resolved up to $\nu=14$ (except $b^3\Sigma_u$, which is repulsive). Note that depending on the how the next few weeks go, more reactions can be added. 

\begin{itemize}
    \item Molecular charge exchange from $X^1\Sigma_g$;
    \item Dissociative attachment from $X^1\Sigma_g$ and $B^1\Sigma_u$;
    \item Vibrational transitions (collisional excitation and deexcitation) in $X^1\Sigma_g$ and $B^1\Sigma_u$;
    \item Dissociative excitation from $X^1\Sigma_g$;
    \item Ionization from $X^1\Sigma_g$, $B^1\Sigma_u$, $C^1\Pi_u$, $EF^1\Sigma_g$, $a^3\Sigma_g$ and $c^3\Pi_u$;
    \item Collisional excitation and deexcitation between (cross sections for deexcitation calculated using the detailed balance principle): 
    \begin{itemize}
        \item $X^1\Sigma_g \leftrightarrow B^1\Sigma_u$;
        \item $X^1\Sigma_g \leftrightarrow C^1\Pi_u$;
        \item $X^1\Sigma_g \leftrightarrow EF^1\Sigma_g$;
        \item $X^1\Sigma_g \leftrightarrow a^3\Sigma_g$;
        \item $X^1\Sigma_g \leftrightarrow c^3\Pi_u$;
        \item $X^1\Sigma_g \leftrightarrow d^3\Pi_u$;
        \item $B^1\Sigma_u \leftrightarrow C^1\Pi_u$;
        \item $B^1\Sigma_u \leftrightarrow EF^1\Sigma_g$;
        \item $C^1\Pi_u \leftrightarrow EF^1\Sigma_g$;
        \item $a^3\Sigma_g \leftrightarrow d^3\Pi_u$;
        \item $c^3\Pi_g \leftrightarrow d^3\Pi_u$;
    \end{itemize}
    \item Radiative deexcitation:
    \begin{itemize}
        \item $B^1\Sigma_u \rightarrow X^1\Sigma_g$;
        \item $C^1\Pi_u \rightarrow X^1\Sigma_g$;
        \item $EF^1\Sigma_g \rightarrow X^1\Sigma_g$;
        \item $EF^1\Sigma_g \leftrightarrow B^1\Sigma_u$;
        \item $EF^1\Sigma_g \leftrightarrow C^1\Pi_u$;
        \item $a^3\Sigma_g \rightarrow b^3\Sigma_u$ (dissociation);
        \item $a^3\Sigma_g \leftrightarrow c^3\Pi_u$;
        \item $d^3\Pi_u \rightarrow a^3\Sigma_g$
    \end{itemize}
    \item Reactions with D$_2^+$:
    \begin{itemize}
        \item $e+\text{D}_2^+\rightarrow 2\text{D}$;
        \item $e+\text{D}_2^+\rightarrow e + \text{D}^++\text{D}$;
        \item $e+\text{D}_2^+\rightarrow 2e+2\text{D}^+$;
    \end{itemize}
    \item Reactions with D$^-$:
    \begin{itemize}
        \item $\text{D}^++\text{D}^-\rightarrow 2\text{D}$;
        \item $\text{D}^++\text{D}^-\rightarrow e + \text{D}^++\text{D}$;
    \end{itemize}
\end{itemize}

The fully vibrationally resoled model allows us to model the vibrational distribution of not only the ground state, but the excited states as well. The distribution of the $d^3\Pi_u$ state is particularly interesting, because the transition between the $d^3\Pi_u$ and $a^3\Sigma_g$ produces measurable and visible emission. It is therefore interesting to compare the calculated distribution to experiment. 

Additionally, this model allows us to calculate the radiative losses of the molecules accurately. 

\subsection{Verification of the model using detailed balance}
First, we would like to verify that the model does indeed produce the expected result in certain simple cases. We will first restrict ourselves to the case that only collisional vibrational transitions are added (see equation \eqref{eq:rea_vibr_trans}. We can calculate the vibrational distribution as a function of temperature. We can also fit the vibrational distribution to the according to equation \eqref{eq:bolzmann}. We use the following function to fit the distribution as a function of energy:
\begin{equation}
    f(x) = c_0e^{c_1x},
    \label{eq:Bolzmann_fit}
\end{equation}
where $c_0$ and $c_1$ are fit constants. \autoref{fig:Bolzmann_proof} contains plots of the vibrational distribution as well as a plot containing $c_1$ as a function of temperature. 

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/Bolzmann_fit.png}
         \caption{Vibrational distribution.}
         \label{fig:Bolzmann_fit}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/Inv_decay_const.png}
         \caption{$\frac{1}{c_1}(T)$}
         \label{fig:Inv_decay_constant}
     \end{subfigure}
        \caption{(a) contains a plot of the vibrational distribution in the ground state of D$_2$ for two different temperatures. The distributions form straight lines as a function of energy, which indicates that the densities indeed follow the Bolzmann distribution of \eqref{eq:bolzmann}. (b) contains a plot of the inverse of the fit constant $c_1$ (see \eqref{eq:Bolzmann_fit}) as a function of temperature. $1/c_1$ appears to be proportional to T, which again confirms that the population fractions indeed follow a Bolzmann distribution.}
        \label{fig:Bolzmann_proof}
\end{figure}





\subsection{Distribution in $d^3\Pi_u$}
Using the vibrationally resolved model, the distributions of the ground state, as well as the excited states can be modelled. This allows for the calculation of emission spectra for any transition between electronic states of D$_2$. 

An important diagnostic in divertor plasma spectroscopy makes use of emission from the transition between the $d^3\Pi_u$ and $a^3\Sigma_u$ states. The emission spectrum from this transition depends on the vibrational distribution of the upper electronic state (see equation \eqref{eq:kappa_p}, \eqref{eq:Xeff}). The relative populations of the vibrational levels in the $d^3\Pi_u$ state can be calculated in two ways. 

The distribution can be obtained by using Franck-Condon factors to map the ground state distribution to the upper state. The advantage of this method is that there is no need to model the upper state, you only need the ground state distribution to calculate the populations in the upper state. Since the ground state distribution is only very weakly affected by the distributions in high electronic states, modelling them is unnecessary. 

The second method is to directly calculate the populations in the upper state using the model. It is necessary to include many different vibrationally resolved excited states, because the distribution in the $d^3\Pi_u$ state is highly influenced by the distributions of all the other states. The advantage of modelling all these states explicitly, in stead of mapping the ground state to the excited state, is that this method is more accurate. 

\autoref{fig:d3_dist} shows the vibrational distribution in the upper state for different temperatures. The figure contains both the distribution calculated using mapping from the ground state, and calculated directly from the model. The mapping closely resembles the calculated distribution for high temperatures, but deviates for lower temperatures. This indicates that there are processes at lower temperatures that are not taken into account by the mapping, and it is therefore necessary to model the excited states vibrationally resolved at these temperatures. 

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/d3_dist_low.png}
         \caption{$Te = 0.1$}
         \label{fig:d3_dist_low}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/d3_dist_high.png}
         \caption{$Te = 100$}
         \label{fig:d3_dist_high}
     \end{subfigure}
        \caption{Vibrational distribution in the $d^2\Pi_u$ state at different temperatures. $n_{d3,v}$ is the density of molecules in the $d^3\Pi_u$ state with vibrational quantum number $v$, and $n_{d3}$ is the total density of molecules in the $d^3\Pi_u$ state. The Franck-Condon mapping is quite close to the modeled distribution for higher temperatures, but deviates more at lower electron temperatures.}
        \label{fig:d3_dist}
\end{figure}

\newpage

\subsection{Emission spectra}
As previously stated, the vibrationally resolved model allows us to calculate the vibrational distributions in the electronically excited states. This also enables us to calculate effective emission rate coefficients of equation \eqref{eq:Xeff}. By calculating $X_{eff}$ as a function of photon energy, a spectrum can be generated. The emission spectrum in the Fulcher band ($d^3\Pi_u$ to $a^3\Sigma_g$) is of particular experimental interest. \autoref{fig:Spectra} contains several different emission spectra at different temperatures. \autoref{fig:Spectr_3.3} and \autoref{fig:Spectr_100} contain the total emission from every transition in the model. \autoref{fig:Spectr_Fulcher_01} and \autoref{fig:Spectr_Fulcher_100} contain emission only from the $d^3\Pi_u$ to $a^3\Sigma_g$ transition.

\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/Spectr_303.png}
         \caption{Total emission spectrum.}
         \label{fig:Spectr_3.3}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/Spectr_100.png}
         \caption{Total emission spectrum.}
         \label{fig:Spectr_100}
     \end{subfigure}
          \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/Spectr_Fulcher_01.png}
         \caption{Fulcher band emission spectrum.}
         \label{fig:Spectr_Fulcher_01}
    \end{subfigure}
         \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/Spectr_Fulcher_100.png}
         \caption{Fulcher band emission spectrum.}
         \label{fig:Spectr_Fulcher_100}
     \end{subfigure}
        \caption{Emission spectra for different temperatures. (a) and (b) contain the total emission from all the different radiative transitions in the model. (b) and (c) contain only the emission from the $d^3\Pi_u$ to $a^3\Sigma_g$ transition. You can see that different wavelengths of emission will dominate at different temperatures. Also note that $X_{eff}$ is much lower for $T_e = 0.1$ eV than for 100 eV. }
        \label{fig:Spectra}
\end{figure}


\subsection{Radiative power losses.}
The main objective of this paper is to accurately model the plasma in a divertor in the detached regime. As stated in the introduction, plasma-molecular interactions in detached plasmas can cause significant radiative power losses. Using the current model, the effective power loss rate coefficient $P_{eff}$ can be calculated. \autoref{fig:Power_loss} contains $P_{eff}$ as a function of temperature. The $B^1\Sigma_u\rightarrow X^1\Sigma_g$ and $C^1\Pi_u\rightarrow X^1\Sigma_g$ transitions together cause over 95\% of the total radiative power loss of the system. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Pictures/Power_loss.png}
    \caption{Radiative power loss for different transitions as a function of temperature. The $B^1\Sigma_u\rightarrow X^1\Sigma_g$ and $C^1\Pi_u\rightarrow X^1\Sigma_g$ transitions are shown, because these two transitions cause over 95\% of the total radiative power loss.}
    \label{fig:Power_loss}
\end{figure}

\subsection{MAR, MAD and MAI}
The model can also be used to calculate effective rates for different molecular processes in the plasma. In particular Molecular Activated Recombination (MAR), Molecular Activated Dissociation (MAD) and Molecular Activated Ionization (MAI) are interesting. These reactions can occur either through creation of $D_2^+$ or $D^-$ ions. \autoref{fig:ion_densities} contains a plot of the normalized densities for both ion species, and \autoref{fig:MA_rates} gives the rates of MAR, MAD and MAI as a function of temperature, also for both ion species.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/D_ions_dens.png}
         \caption{Ion densities.}
         \label{fig:ion_densities}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Pictures/MA_reactions.png}
         \caption{Effective rate coefficients}
         \label{fig:MA_rates}
     \end{subfigure}
        \caption{(a) contains the ion density normalized by the molecular density $n_0$, for both $D^-$ and $D_2^+$ ions. (b) contains a plot of the effective rate coefficients for MAR, MAD and MIE, also for both ion species.}
        \label{fig:MA_info}
\end{figure}

\section{Update results 12-6-2023}

\subsection{Vibrational-vibrational exchange}
Thus far, only reactions involving one background species, and one regular species have been considered. However, especially in plasmas with high molecular density, collisions between molecules might be important. In particular Vibrational-Vibrational Exchange (VVE), can potentially influence the vibrational distribution in the ground state. The reaction formula for VVE is given below.

\begin{equation}
    \text{D}_2(X^1\Sigma_g,v)+\text{D}_2(X^1\Sigma_g,w+1)\rightarrow\text{D}_2(X^1\Sigma_g,v+1)+\text{D}_2(X^1\Sigma_g,w),
    \label{eq:VVE}
\end{equation}
$\text{D}_2(X^1\Sigma_g,v)$ are deuterium molecules in the electronic ground state with vibrational quantum number $v$, with $v>w$.

The problem is that these reactions involve two deuterium molecules, and are therefore quadratic in $n_0$. It is therefore not possible to linearize equation \eqref{eq:Rate_eq}, and write it as equation \eqref{eq:matrices}. It is possible, however to obtain an approximate steady-state distribution including VVE by using an iterative approach. 

In stead of solving the linear system of \eqref{eq:matrices} directly for steady state, we evolve the density distribution time dependently with some time step $\tau$. We first solve the linear system of equations (equation \eqref{eq:matrices}) without VVE. This gives us an initial density profile $\mathbf{n}$ we can use to calculate the VVE reaction rates.

\begin{equation}
    R^{v,v+1}_{w+1,w} = n_vn_{w+1}k^{v,v+1}_{w+1,w},
\end{equation}

Where $R^{v,v+1}_{w+1,w}$ is the reaction rate (in cm$^{-3}$s$^{-1}$), $n_v$ is the density of $\text{D}_2(X^1\Sigma_g,v)$, and $k^{v,v+1}_{w+1,w}$ is the reaction rate coefficient (in cm$^3$s$^{-1}$) of equation \eqref{eq:VVE}. Using these rates, we can calculate an additional source vector $\pmb{\Gamma}_\Delta$, which represents the particle sources and sinks as a result of VVE. The components $\Gamma_{\Delta}^v$ are given by
\begin{equation}
    \Gamma_{\Delta,v} = -\sum_{w=0}^{v-1}R^{v,v+1}_{w+1,w} + \sum_{w=0}^{v-1}R^{v-1,v}_{w,w-1}.
\end{equation}
Using $\pmb{\Gamma}_\Delta$, we evolve the distribution up to $t=\tau$, using the following adapted equation. 
\begin{equation}
    \dot{\textbf{n}} = \textbf{M}\textbf{n}+\pmb{\Gamma}+\pmb{\Gamma}_\Delta.
\end{equation}
The densities $\mathbf{n}$ we get from this equation can then be used to calculate the new $\pmb{\Gamma}_\Delta$, and repeat the process. This procedure is done until the densities converge to constant values. This way we can obtain a steady state distribution of the model including VVE. 

The rate constants used for VVE are calculated using a formula from (...).

\begin{equation}
    k^{v,v+1}_{w+1,w} \approx (v+1)(w+1)k^{0,1}_{1,0}\left(\frac{3}{2}-\frac{1}{2}e^{-\delta(v-w)}\right)\exp(\Delta_1(v-w)-\Delta_2(v-w)^2),
\end{equation}
with $k^{0,1}_{1,0}\approx4.23\cdot10^{-15}(300/T)^{1/3}$ cm$^3$s$^{-1}$, $\delta\approx 0.21(T/300)^{1/2}$, $\Delta_1\approx0.236(T/300)^{1/4}$, and $\Delta_2 \approx 0.0572(T/300)^{1/2}$. Here $T$ is the temperature of the D$_2$ molecules in Kelvin. 

\subsection{Comparing calculated rates to AMJUEL database. }


\subsection{Vibrational-translational relaxation.}

Another way that molecules can change their vibrational state is by collisions with atomic deuterium. This is the main path for vibrational energy losses in the plasma. In this reaction, vibrational energy is transferred to translational energy of the atom and molecule, and is therefore called Vibrational-Translational (VT) relaxation. 


\begin{equation}                                  \text{D}+\text{D}_2(X^1\Sigma_g,v)\rightarrow\text{D}+\text{D}_2(X^1\Sigma_g,v\pm1)
    \label{eq:VVE}
\end{equation}
